Temporal Consistency Loss for High Resolution Textured and Clothed 3DHuman Reconstruction from Monocular Video

We present a novel method to learn temporally consistent 3D reconstruction of clothed people from a monocular video. Recent methods for 3D human reconstruction from monocular video using volumetric, implicit or parametric human shape models, produce per frame reconstructions giving temporally inconsistent output and limited performance when applied to video. In this paper, we introduce an approach to learn temporally consistent features for textured reconstruction of clothed 3D human sequences from monocular video by proposing two advances: a novel temporal consistency loss function; and hybrid representation learning for implicit 3D reconstruction from 2D images and coarse 3D geometry. The proposed advances improve the temporal consistency and accuracy of both the 3D reconstruction and texture prediction from a monocular video. Comprehensive comparative performance evaluation on images of people demonstrates that the proposed method significantly outperforms the state-of-the-art learning-based single image 3D human shape estimation approaches achieving significant improvement of reconstruction accuracy, completeness, quality and temporal consistency.

==> Experiments_old.tex <==
\section{Experiments}\label{Sec:Exp}


% Don't forget: PIFUHD hallucinates a lot. show it. It hallucinates details which are not there. for example texting and walking data. 
% PIFUHD hallucinating different 3D per frame, without any temporal consistency. 
% for example, subject is walking, however, 3D model is all same pose. 

% Ayrica, voxel oldugu icin intermediate representaiton, shape i encode edebiliyoruz ve bu bize hem geometry hem de texture da isimize yariyor. 

% Comparison section: -> we compare our method other implcit reconstruction methods, whose code is available. 

% our proposed method, since voxel encoding, can estimate the invisible side of the texture and geometry well. -> use texting data. 

% In the experiments, we fine tune the pifu, but trainign code for PIFUHD was not available. 

% Pifu fine tuned however, main dataset has mostly stainding pose human. so there is bias fo that. also, in Fig, X, geometry prediction is is not temporal consistent. -> bunlari cembere alalim. For example, every frame, pifuhd predicts different face reconstruction. Pifu predicts incosistent reconstruction as well. 

% show consistency in texture and geometry   -> and show inconsistnecy in texture (PIFU)

% BUff -> we used the trained network on synthetic data diyelim. 

% In the experiemtns, especially video, we will show that even if we proces them frame by frame, the results are temporally coherent. Walking den bir data alalim. ve onu yandan gosterleim. bu guzel olur. 

%% Comparison'a eklenecek. -> elimdeki 4 video dan yapalim bunu. daha artirmayalim. 
% Kesin yapalim: - absolute relative temporal error - diye bir sey varmis. buna bakalim. bu paperda: https://arxiv.org/pdf/2001.02613.pdf . bunu bizim paper a uyarlayalim. yani relative temporal error u hem geometry hem de texture da gosterelim. -> bir tane gorsel ya da grafik yapacagiz, ve temporal loss olmadan ve olarak, nasil temporal consistency i artirdigini gosterecegiz. ya da bizim metodu diretk baska temporal consistency olmayan metodla karsialstirip da yapabilriz. dusun bunu. 
% Modelleir sadece single frame gibi gostermeyelim, video boyunca run edelim.
% Diger metodlarla da compare ederken boyle yapalim. onemli olan consistency falan gostermek. 

% invisible regionlari gosterelim. onlarla da karsilastiralim. 

% TODO: 
% comprasionda, 3D reconstruction quality karsilastir bir de, arbitrary pose icin sonucu karsilastir. burdan vuracagiz. Bir de texture karsilastir. 
% Sonuclari gosterirken, deftere cizdigim sekli yapalim. 3D modeller (geo ve texture) altinda da video frames olsun. 

% Analyse the experiemtns based 
% - 3D reconsturciton and 3D surface accuracy and completeness fro arbitrary poses
% - Quality of textures 

% Ablation: 
% - hwo about the perfomance of hybrid decoder, even if voxel is coarse? I mean not accurate? 
% - draw the convergence graphs of proposed decoder and pifu, 

% Gozlem: voxel 3d iyiyse 3d reconstruction daha  iyi mi oluyor? buna bak. 

%% Once resultlari koyalim, sonra comparisonlari koyalim. 

% Here, compare our method with other in terms of geometry and texture details. not only for single image, but also for video and consistency manner. We will show that our method is better for temporal coherency and reconstru tion quality of fully texrtured 3D. 


% if-net metoduyla bizim refinement i karsilastiralim. bizimle if=net i karsilastiralim koyalim sonuc. kesin. bizimki daha iyi yapacaktir cunku daha cok info veriyoruz feature embdggin de. 


% Temporal olarak hatanin nasil degistigini gosterelim farkli metodlarla. bu onemli. 


% Resultlari gosterrirken, yandan da goster. hareketi gorelim yani. 


% Datasetleri tanitalim. traiign test splitleri nasil ayirdik anlatalim. 

% Experiment da, wide time frame seperated frames i incleyelim. farkli thresholdda koyalim. ya da bir tanesini motion threshold ile yapalim. bir tanesini butun framelere uygulayalim ve farklarini gorelim. Bir de kac tane view dan hesapladik 'temporal consistency' loss u onun da ablation i olacak. 


% We are learning temporal coherent features, so, our proposed network gives us coherent 3d recons. 

% Hao li eccv 2020, monocular human volumetric real time captrue paper kodu var denenecenk. 

% We also provide the BUFF renderings. 

% Temporal voxel de SGD optimizer kullandik, fakat implicti geometry ve texture da ise prop optimizer kullandik. 

% Vibe ile karsilastiriken, onun simplfy temporal ini calistiralim. bundan da bahsedelim paperda. 

% BAK BUNA: Temporal coherency i nasil gosteriyor paperlar? sonuclari? bakalim buna. ben bir plot cizerim. 


% Pifu ve Pifu HD nin arbitray pose lari handle edemedigni gosterleim ve temporal consistency ni olamdingi gosterelim. bunu nedeni onerdigimiz loss function. ve topology i voxel iel korumamiz. 

%ablation
%- voxel size i degistir ve yap.
%- decoder i degistir
%- time i degistir. temporal consistency icin. 
%- Decoder a septh degil sadece image features ve voxel koyalim. 

% Voxel refinement icin su iki metodla karsilastiracagiz: \cite{peng2020convolutional,chibane2020implicit}


\subsection{Implementation Details}
% First we train the voxel network and then implicit function decoder for geoemtry and texture respectively.
% network u nasil train ediyoruz. kac epoch ile, nasil optimize ettik? nasil normalize ettik. 

% details of network with decoder details will be available in supplementary document. 


% Comparioson with other methods, 
% ARCH paperinin pifuyu yerdigi gorselleri kullanalim. ve arch in sonuclarini da buradan kopyalalalim. yani image leri. ve diyelim ki bizim 3D imiz cmparable ve texture imiz daha iyi arbitrary pose icin. Texture reconstrucitoni daha iyi oldugunu dusunuyoruz diyelim. 


% implementationda, sundan da bahsedelim: 3D occupancy network sonucunu marching cube ile mesh yapiyoruz diyelim. 

% -> which image encoder we used? for geometry and texture. bunlari yazalim buraya. % Geometry -> shape encoding var, bir de hourglass network var image feature lar icin
% Texture -> shape encoding var, bir de resnet var image feature lar icin


% Bir yerde, sampling i anlatacagim. -> bence burda anlatalim. ve diyelim mi, samplingi de kolaylastiriyorz diyelim bu voxel intermediate representation. 

% implicit network u secerken sigma yi nasil sectik ve kac tane sampled point aldik yazalim. 


% FUTURE WORK: -> We will explore hybrid representations more. for better implciti reconstruction. 

==> Method_old.tex <==
\section{Temporally Consistent Textrued 3D Human Reconstruction from a Video}
%
This section explains the novel proposed method for temporally consistent textured 3D human reconstruction from a monocular video, illustrated in Fig. \ref{fig:geometry_network} - \ref{fig:texture_network}. Fig. \ref{fig:geometry_network} and \ref{fig:texture_network} shows temporally consistent training for 3D human surface reconstruction and texture prediction respectively. A monocular video of a dynamic human with arbitrary pose, clothing, and viewpoint is given as input to the pipeline, and the network predicts the 3D voxelized outputs, 3D occupancy probabilities and 3D texture values for 3D reconstruction. 

In contrast to previous single-view 3D reconstruction approaches, Table \ref{table:Rel_method_comp}, the proposed method is trained using novel loss functions on time distant frames of a dynamic human, as shown in Fig. \ref{fig:geometry_network} - \ref{fig:texture_network}. Each video frame is passed through its own voxel regression network and parameters are shared between the networks. 
The proposed voxel regression network learns to reconstruct human shape in a temporally consistent manner. The predicted voxel reconstruction is then passed to the proposed hybrid implicit surface function decoder to predict occupancy values for 3D points. Then, texture prediction network takes the extracted features from the output of implicit surface function network and predicts the color of visible and invisible points in a temporally consistent manner. The error between the estimated 3D voxel occupancy and ground-truth 3D models is computed for each time frame, and time-dependant 3D occupancy grids are transformed from one frame to other frames using temporal correspondence to evaluate the temporal consistency loss for occupancy. The loss term enables the network to learn feature extraction robust to temporal changes and to predict temporally consistent 3D human reconstruction. In the context of high level of surface details, voxel representation is limited even if this representation reduces the irregularity and improves the locality for 3D reconstruction. So, the proposed hybrid implicit surface function decoder improves the level of surface details using the features extracted from 3D voxel, input image and depth. The error between estimated 3D point occupancy and ground-truth 3D models is computed for each time frame. For texture prediction, each video frame is passed through its own texture decoder and parameters are shared between the networks. The error between the estimated and the ground-truth colors is computed for each time frame, and time-dependant color values are transformed from one frame to other frames to using temporal correspondences to evaluate the temporal consistency loss for color. The proposed network is scalable to \textit{N}-frames, and to various voxel resolution.
%[ADD] Should I add -> , and a detailed ablation study on the performance of the network with number of frames and 

% however, this voxel gives the topology of the shape, in the second stage, we use the novel implicit function bla bla. Difference between geopifu and our network will be explained in Learnign architecrure part. 
% Voxeli yapmamizin nedeni ne? Neden temporal consistency i implicit de yapamiyoruz? 

% hybrid representation a odaklan. 

% Kullanilan devoderlari (geopifudan farkini falan) falan, 'Learnign Architecture' da aciklayalim.
% Loss functionlari ayri baslikta yazalim. 

% Overall method 
% Koda bakarak cizelim diagram i. 

% ARCh paper notation kullanalim. 

%What we propose in general: hybrid loss function which includes gt loss and temporal loss. 
% su paperdan esinlenelim: http://forestlinma.com/welcome_files/hzhuang_CVPR_2017.pdf


%\subsection{3D Human Representation}
%\label{sec:human_repres}


\subsection{Learning Architecture}
\label{sec:learning_arch}

% Say that network is end-to-end because, we compute the 3D geometric features form the predicted occupancy values, (bot after marching cubes). 
% N tane ye cikabilir network, cunku, voxel ne kadar coarse olsa da memory consumption az oluyor, ve coarse u halledebiliyoruz. bir de implicit decoder texture icin N tane frame e de cikabiliyor. 

% Neden voxel de yaptigimizi temporal consistency burada anlatalim. network un train edilmesi geregi positive ve negative sampling pairlardan. 

The proposed learning architecture is illustrated is illustrated in Fig. \ref{fig:geometry_network} - \ref{fig:texture_network}. The proposed architecture consists of three sub-networks. Inspired by previous works \cite{newell2016stacked,caliskan2020multi}, we use stack hourglass network architecture with skip connections for  \textit{Temporal Voxel Regression Network (TRVN)}. The learning architecture 
consists of multiple parallel stacked hourglass networks with shared parameters. This architecture allows the introduction of temporal loss function. Image, $I$, input is passed through this \textit{image-to-volume} network, $\mathcal{G}$, and \textit{TRVN} predicts the voxel occupancy volume: $V$ =  $\mathcal{G}(I)$, $V \in \mathbb{R}^{N \times N \times N }$ where $N \in \mathbb{N}$ denote the input resolution. Inspired by previous works \cite{saito2019pifu}, the second sub-network, \textit{Hybrid Implicit 3D Reconstruction}, i.e. \textit{geometry prediction network}, learns to predict implicit surface function, $f_{geometry}(.)$. In contrast to previous implicit surface function networks \cite{saito2019pifu,saito2020pifuhd,huang2020arch}, the proposed decoder takes not only pixel-wise image features but also point-wise shape encoding from temporal consistent voxel occupancy volume. In particular, the proposed hybrid implicit network consists of point-wise 3D voxel encoder, $\mathcal{S}(.)$, pixel-wise image encoder, $\mathcal{H}(.)$, and depth encoder, $\mathcal{D}(.)$, and passes these features through implicit surface function decoder, $f_{geometry}(.)$. We use multi-scale 3D shape encoder \cite{chibane2020implicit}, which is a rich encoding of data, $V$, through subsequently convolving it with learned convolutions. It is the first to use this shape encoding for single-view textured 3D human reconstruction in the context of hybrid representation. Shape decoder, $g(V) := F_1, F_2, \dots F_n$, is defined as combination of deep feature grids, $F$, for $n$ number of stages. In the early stages features grids capture high frequency details, and receptive fields increases for high level of stages to capture global 3D structure. For a 3D point, $\mathbf{X}$ and its 2D projection, $\mathbf{x} = \pi( \mathbf{X})$, the proposed hybrid decoder takes inputs as multi-scale shape encoding, $\mathcal{S}(\mathbf{X}) = [F_1(\mathbf{X}),F_2(\mathbf{X}) \dots F_n(\mathbf{X}) ]$, an pixel-wise image features, $\mathcal{H}(I(\mathbf{x}))$, and depth encoding, $\mathcal{D}(\mathbf{X})$, and pass them to Multi Layer Perceptron (MLP) to predict occupancy value for the point, $\mathbf{X}$:

\begin{equation} \label{eq:hybrid_geometry_dec}
f_{geometry}(\mathcal{S}(\mathbf{X}), \mathcal{H}(I(\mathbf{x})), \mathcal{D}(\mathbf{X}) ) = s : s \in \mathbb{R}, s \in [0,1]
\end{equation}

For the third sub-network, \textit{texture prediction network}, we use another hybrid decoder, $f_{color}(.)$ which predicts the color, $C(\mathbf{X})$, for a 3D point, $\mathbf{X}$, on the surface of the reconstruction. In particular, the proposed hybrid color network consists of point-wise 3D shape encoder, $\mathcal{S}(.)$, pixel-wise image encoder, $\mathcal{H}(.)$, and depth encoder, $\mathcal{D}(.)$, and passes these features through implicit color function decoder, $f_{color}(.)$. Different from \textit{geometry prediction network}, multi-scale shape encoder takes input as the output of \textit{geometry prediction network}, which is point-wise occupancy predictions. \textit{Color prediction decoder} is formalized as:

\begin{equation} \label{eq:hybrid_color_dec}
f_{color}(\mathcal{S}(\mathbf{X}), \mathcal{H}(I(\mathbf{x})), \mathcal{D}(\mathbf{X}) ) = c : c \in \mathbb{R}^{3\times1}
\end{equation}

In contrast to previous approaches \cite{huang2020arch,saito2019pifu}, hybrid decoder captures the global topology of the shape with the shape encoding to predict accurate geometry and texture for 3D reconstruction. In overall network, we propose an end-to-end neural network architecture to learn temporally consistent 3D textured human reconstruction from a video. The details of the image encoders and MLP networks are explained in  Sec. \ref{Sec:Exp}. 


% [ADD] -> if the overall network is end-to-end, please state it in this section.
% [ADD] Do we need to explain shape decoder? I think so. 
% [ADD] -> Should I add encoder architecture's diagram here ? 
% [ADD] -> The details of network architecture is provided in supplementary documents.
% [Add] -> Should I add more about geopifu here? I already mentioned it in related work? 

%% !!! Buldum geopifuyu nasil atlatacagimi !!!
% It may seem that geopifu's hybrid network resembles the our hybrid reconstruction, however, they are differetn : explain. and also, we are not proposing hybrid imlict for geometry, but also texture in a temporal consistent manner. 
% Enson burayi acikla. 
% Geopifu ile de onerdigmiz metodun hybrid implicit 3D reconsturction parti formulize edilebilir, fakat, as it is stated in [REF to ifnet paper] -> 
% Ifnet paperinda, 3.1 ve 3.2 de, latent voxeli kullanmakla, ifnetin convolution based metodunu kullanmak karsilastiriliyor. -> buna gore, 1-) geopifu gibi latent feature lari kullanmak complex geometry i, like articulated geometry, aciklamakta yetersiz kaliyor, 2-) latent feature approaches do not preserve details on 3D surface. 
% Bu yuzden biz de novel bir combination of convolved features from 3D shape, and pixelwise image features and depth encoder. -> this is new.
%% !!! Buldum geopifuyu nasil atlaatacgimi !!!
% Difference between GeoPIFU -> 
% The proposed hybrid implicit 3D reconstruciton may seem to similar to GeoPIFU; however, 3D shape encoder parts are different. We use the shape encoding proposed in \cite{chibane}, and modify it for single-view 3D human reconstruction. Instead of usign latent voxel features [Ref to Geopifu], !!! we prefer to learn the shape encoding which is the 3D convolution of 3D point on the voxels, which are trainable !!! (Cok onemli burasi)
% And proposed method is the first mehtod that combines these shape encoding and image features. -> ifnet i iyi oku. 

\begin{figure}[!ht]%[hb]%[H]
\begin{center}
\includegraphics[width=\columnwidth]{latex/images/Method_Diagram_corr.001.png}
\caption{Temporal 3D vertex correspondences between time distant frames from a video}
\label{fig:temporal_corr}
\end{center}
\end{figure}

\subsection{The Proposed Loss Functions}
\label{sec:loss_func}


The proposed learning architecture is supervised from the ground-truth 3D human models rendered from temporal frames and self-supervised between time distant frames from a monocular video. In order to train the \textit{temporal voxel regression network}, the 3D loss function $\mathcal{L}_{3D}^{Voxel}$ computed the error between the estimated 
3D voxel occupancy grid ($\hat{V}_t$) and 3D ground-truth ($V_t$) for time frame $t$. As stated in Equation \ref{eq:l_3D_1}, the binary cross entropy \cite{jackson2017large} is computed after applying a sigmoid function on the network output. In particular, we used weighted binary cross entropy loss and $\gamma$ is a weight to balance occupied and unoccupied points in the voxel volume:


\begin{equation} \label{eq:l_3D_1}
\mathcal{L}_{3D}^{Voxel} = { \sum_{t=1}^{N}  \mathcal{L}( \mathcal{V}_{t}, {\hat{\mathcal{V}}_{t}} ) }
\end{equation}
%
\begin{gather*} \label{eq:l_3D_2}
\mathcal{L}( \mathcal{V}_{t}, {\hat{\mathcal{V}}_{t}} ) = \\ {\sum_{x} \sum_{y} \sum_{z} \gamma\mathcal{V}_{t}^{xyz}\log{{\hat{\mathcal{V}}_{t}}^{xyz}} + (1-\gamma)(1-\mathcal{V}_{t}^{xyz})(1-\log{{\hat{\mathcal{V}}_{t}}^{xyz}}) } 
\end{gather*}
where ${\mathcal{V}}^{xyz}$ stands for occupancy value of a voxel grid, ${\mathcal{V}}$, at position $(x,y,z)$. Training a network with only binary cross entropy loss gives temporally inconsistent reconstruction quality for the dynamic parts of the human body as shown in Fig. \ref{fig:geometry_network}. In order to improve 3D model accuracy and completeness, we propose a second loss function, \textit{temporal consistency loss} ($\mathcal{L}_{TC}$) between multiple video frames of the same subject. With the \textit{temporal consistency loss}, the propose representation can learn features robust to temporal changes, self-occlusion and flickering between frames. 3D voxel occupancy grids estimated per frame and the temporal correspondences between vertices are transformed to voxel correspondences, Fig. \ref{fig:temporal_corr}. The \textit{temporal consistency loss} is defined in Equation \ref{eq:l_TC_1}, $L2$ loss is computed between voxel occupancy estimates, $\hat{V}$, from one time frame and $N-1$ other frames.

\begin{equation}\label{eq:l_TC_1}
\mathcal{L}_{TC}^{Voxel} = \sum_{t=1}^{N} \sum_{\substack{l=1\\  l \neq t }}^{N} {\hat{\mathcal{L}}(\hat{\mathcal{V}}_{t}, \hat{\mathcal{V}}_{l} )}
\end{equation}
%
\begin{equation*}
\hat{\mathcal{L}}( \hat{\mathcal{V}}_{t}, {\hat{\mathcal{V}}_{lj}}) = \sum_{x} \sum_{y} \sum_{z} { \lVert \hat{\mathcal{V}}_{ij}^{xyz} - \hat{\mathcal{V}}_{l}^{\mathcal{P}(xyz)} \rVert }_{2}
\end{equation*}
where $\mathbf{\mathcal{P}}$ is the transformation operator between 3D point correspondences. 

In order to train implicit surface function decoder, \textit{Hybrid Implicit 3D Reconstruction Network} takes 3D point samples around the surface of 3D human models and their occupancy values. To create training point samples, we sample a number $n \in \mathbb{N}$ of points $\mathbf{p}_{i} \in \mathbb{R}^3, i \in 1,\dots,n$ by sampling points on the ground-truth surfaces for every 3D human model, and adding random displacements $\mathbf{n}_i \sim \mathcal{N}(0,\sigma)$, i.e. $\mathbf{p}_{i}^{s} := \mathbf{p}_i + \mathbf{n}_i$. Then we compute the ground truth occupancy values of the sampled points, $o(\mathbf{p}_i^s) \in \{ 0,1\}$. If $\mathbf{p}_{i}^{s}$ is inside mesh surface, the corresponding $o(\mathbf{p}_i^s) = 1$ and if not, $o(\mathbf{p}_i^s) = 0$. We train the \textit{geometry prediction network} (Equation \ref{eq:hybrid_geometry_dec}) by minimizing the average of mean squared error: 

\begin{equation}\label{eq:l_HGeo_1}
\mathcal{L}_{3D}^{Hybrid} = \frac{1}{n} \sum_{i=1}^{n} {\lVert f_{geo}(\mathcal{S}(\mathbf{X_i}), \mathcal{H}(I(\mathbf{x_i})), \mathcal{D}(\mathbf{X_i}) ) - o(\mathbf{X_i}) \rVert}_2
\end{equation}

We train \textit{texture prediction network} (Equation \ref{eq:hybrid_color_dec}) by minimizing two loss functions, namely $\mathcal{L}_{Color}^{Hybrid}$ and $\mathcal{L}_{Color}^{temporal}$. In order to compute $\mathcal{L}_{Color}^{Hybrid}$, we sample a number $m \in \mathbb{N}$ of points $\mathbf{p}_{i} \in \mathbb{R}^3, i \in 1,\dots,m$ by sampling points on the ground-truth surfaces for every human model. Then, we get the color values of the sampled points, $c(\mathbf{p}_i) \in \mathbb{R}^3$. We train the \textit{texture prediction network} by minimizing the average absolute difference error: 

\begin{equation}\label{eq:l_HText_1}
\mathcal{L}_{Color}^{Hybrid} = \frac{1}{n} \sum_{i=1}^{n} {\left | f_{color}(\mathcal{S}(\mathbf{X_i}), \mathcal{H}(I(\mathbf{x_i})), \mathcal{D}(\mathbf{X_i}) ) - c(\mathbf{X_i}) \right |}
\end{equation}

In order to train texture prediction network in a temporally consistent manner, we use the temporal correspondences of a sampled point, $\mathbf{p}_{i}^{t}$ for $t = \{1,\dots,N-1$\}, and we train the network by minimizing the $L_2$ loss computed between color estimates, $\hat{c}$, from one time frame and $N-1$ other frames


\begin{equation}\label{eq:l_HText_2}
\mathcal{L}_{Color}^{Temporal} = \sum_{i=1}^{n} \sum_{\substack{l=1\\  l \neq t }}^{n} { \lVert \hat{c}(\mathbf{X_i}^{t}) - \hat{c}(\mathbf{X_i}^{l}) \rVert}_2
\end{equation}
%
\begin{equation*}
\hat{c}(\mathbf{X_i})  =  f_{color}(\mathcal{S}(\mathbf{X_i}), \mathcal{H}(I(\mathbf{x_i})), \mathcal{D}(\mathbf{X_i}) ) 
\end{equation*}

The combined loss function is the weighted sum of the all loss functions defined: 

\begin{equation} \label{eq:l_all}
\mathcal{L} = \mathcal{L}_{3D}^{Voxel} + \lambda \mathcal{L}_{TC}^{Voxel} + \mathcal{L}_{3D}^{Hybrid} + \mathcal{L}_{Color}^{Hybrid} + \mu \mathcal{L}_{Color}^{Temporal}
\end{equation}

% Overall loss function is then stated:
% Butun losslari toplayalim sonunda. Total loss u yazalim. 
% Last bir cumle yazalim buraya. 

%\subsection{Temporal Consistency Loss for Geometry and Texture %Prediction}\label{sec:loss_func}


% [ADD] -> Should I mention why we can not implement temporal consistent 3D to implicit but to voxel? 


% Temporal loss u gosterirken, temporal correspondence lari gosterleim figure ile, kucuk  bir figure. Ve sparse correspondence lari kullandigimiz yazalim. Nasil karar verdik hangi frameleri alacagimiza. 


% temporal consistency loss dan bahsederken su paper notatinn ve anlatim kullanalim : https://arxiv.org/pdf/1604.08610.pdf

%In the proposed method, we first introduce the temporal consistency loss for accurate 3D geometry prediction. To do that, we prefer to use voxel 3D representation and using ground-truth correspondences. Temporal consistency loss is not applicable to implicit networks because it is not possible to find 3D correspondences of sampled points. Here we define two loss functions: the first one is the ground-truth loss between predicted and ground-truth voxel occupancies [Eqn XXX]. The second loss is temporal consistency loss between predicted voxel occupancies from multiple consecutive frames. Since ground-truth correspondences of 3D vertices on human body surface are available, we compute the voxel correspondence from them. Based on the voxel correspondences temporal consistency loss is defined in Eqn XXX. In the implementation, frames to be used for temporal consistency loss are selected if the displacement vector between corresponding vertices are above a threshold $\mathcal{\tau}$, and the porposed loss function can be extended to $\mathcal{N}$ number of views. 

%On the other hand, we also propose a method to learn temporally coherent full textured 3D prediction. In order to train the proposed network to learn hybrid representation (Sec. \ref{sec:hybrid_rep}), temporally consistent loss function for 3D texture prediction is introduced. During training of texture prediction network, we are proposing two loss function: Firstly ground-truth loss (Eqn. XXX) between predicted and ground-truth RGB color values of the 3D vertices sampled from the mesh surface. Secondly, temporal  consistency loss is defined as $\textit{L}2$ distance between predicted RGB values for consecutive frames (Eqn. XXX).

% please show the 3D correspondences visually. sparse 3D temporal correspondences. 

% Don't forget to say that, we train the network using widely separated frames. 

% Also mention the silhoutte loss. in voxels

% We are learning temporal coherent features. 

% Temporal consistent 3D geometru ve texture un ayri ayri cizelim diagramlarini. 

% Temporal consistency loss u neden voxel de yapiyoruz? aciklayalim. 

% Temporal consistency loss u implement ederken frkli modellerin voxel sayilari farkli olabiliyor. bunu bir sekilde cozuyoruz. 

% Voxel representationda yaptigimiz temporal loss hesabini detayli anlatalim. nasil buldugumuz mesh correspondencelari ve sonra voxel correspondencelari. 

% Temporal correspondencelari bir gorselle gosterelim. ok cizelim. 

% Calismayan decoder i da koyalim mi. calismayan degil de, farkli decoder olarak koyali sonuclarini gosterelim. bunlarin seklini de cizelim. yani, decoder in seklini. ve sonuc koyalim. bir tane datadan koysak kafi. 


%% IMPORTANT. 
% Soyle desek ya: Multivie consistnecy ye temporal consistency de ekledik. ve bununla beraber bir de hybrid representation getirdik. bunu diyelim.  

%\subsection{Hybrid Representation Learning for Monocular 3D Human Reconstruction}\label{sec:hybrid_rep}

% we propose PVCNN (using implicit funstion decder) that represents the 3D input data in points to reduce thememory consumption, while performing the convolutions in voxels to reduce the irregular, sparse data access and improve the locality -> bunu gibi yazalim. 

% 3D geometry de implicit te temporal consistent voxelden ogreniyoruz. fakat texture da regression oldugu icin burda da temporal loss u ekleyebiliriyoru. UNUTMA. 

% Unutma: during test time, we are sampling around the voxel 3D, this decrease the chance of losing global topology becaue of sampling in Pifu, and PifuHD. 

% GeoPIFU -> Our method and geopifu is different in terms of network structure. ours learns temporal consistent features and learns temporal consistnet 3D geometry. Also, ours learns temporally consistent texture prediction. 
% Difference: Geopifu uses latent voxel features, ours extract scale invariant features from reconstructed temporal consistent voxels. Geopifu does not learn texture. 
% GeoPIFU -> latent space'de P point icin nasil feature extrac ediyor ya? -> biz ise 3D voxel in geometric featureini cikartiyoruz. Yani, predicted 3D voxelden cikartiyoruz.
% Different from GeoPifu, we use another voxel encoder module to extract pointwise feautures from temporally consistent 3D voxel prediction whereas geopifu uses latent voxel feautures from 3D-Unet module in which pointwise feature extraction is not clearly explained in the paper. We also design a texture network and geomety network. 

% For 3D geometry we use the voxel encoder toextract features from voxels, and for texture learning we use another 3D encoder the extract 3D features from 3D reconsturction with high details. And then use them for texture decoder. These geometry encoders are structurally same (details are in supplementatry), but we train two separate encoders in the entrie network. 

% mention hybrid representation and the proposed decoder. 
% Here, explain, our texture difference from Pifu, and our complete network difference from GeoPifu. 

% If-net ten farkli oldugumuz soyleyelim burda. 

% if-net den bahsedelim. If-net in sadece voxel featurelar aldigini soyleyleim. biz ise image ve depth i de aliyoruz. Experimentlerda da gosterelim bizim metod daha iyi gitsin voxelden implciti e, if-net daha kotu gitsin. 

% Deephuman da da voxeli refine etme vra. sonuclari ref edip onun ne kadar kotu yaptigini gosterleim. 

% Computationanl cost and memory footprint of the voxels methods grow cubically wth the 3D resolution. Therefore, we propose a solution to first estiamte temporal conssintet coarse voxel prediction and learnign impliti reocnstruction using the voxel features, iamge features. We call it hybrid representation learning. So, the proposed network is able to reconstruct high resolution 3D geometry and texture. The proposed method is memory and computaton efficient. In the proposed methods, voxels are intermediate 3D representation and the rest of the network learns to predict implicit occupancy values usign voxel features, image features and depth encoding. In Pifu related methods \cite{pifu, pifuhd, arch}, sampling scheme cause lossing the topology of the 3D human. However, it is shown that \cite{caliskan_multiview_consist}, voxel regression keeps the complete toplogy for human to compute 3D for arbitrary pose cases. In the proposed method, voxels are used fot that. 

% Geometry ve texture network u guzel gosterelim. anlatalim, ve fromule edelim.
